Measurement and Analysis of GPU-accelerated Applications with HPCToolkit

To address the challenge of performance analysis on the US DOE's forthcoming exascale supercomputers, Rice University has been extending its HPCToolkit performance tools to support measurement and analysis of GPU-accelerated applications. To help developers understand the performance of accelerated applications as a whole, HPCToolkit's measurement and analysis tools attribute metrics to calling contexts that span both CPUs and GPUs. To measure GPU-accelerated applications efficiently, HPCToolkit employs a novel wait-free data structure to coordinate monitoring and attribution of GPU performance. To help developers understand the performance of complex GPU code generated from high-level programming models, HPCToolkit constructs sophisticated approximations of call path profiles for GPU computations. To support fine-grained analysis and tuning, HPCToolkit uses PC sampling and instrumentation to measure and attribute GPU performance metrics to source lines, loops, and inlined code. To supplement fine-grained measurements, HPCToolkit can measure GPU kernel executions using hardware performance counters. To provide a view of how an execution evolves over time, HPCToolkit can collect, analyze, and visualize call path traces within and across nodes. Finally, on NVIDIA GPUs, HPCToolkit can derive and attribute a collection of useful performance metrics based on measurements using GPU PC samples. We illustrate HPCToolkit's new capabilities for analyzing GPU-accelerated applications with several codes developed as part of the Exascale Computing Project.

==> Makefile <==
generatedfigures=\
	synchronization-eps-converted-to.pdf \
	sparse-output-eps-converted-to.pdf \
	sparse-internal-eps-converted-to.pdf \
	pelec-inst-eps-converted-to.pdf \
	infrastructure-eps-converted-to.pdf \
	hpcviewer_trace-eps-converted-to.pdf \
	hpctoolkit-quicksilver-eps-converted-to.pdf \
	hpctoolkit-eps-converted-to.pdf \
	gpu-cct-eps-converted-to.pdf \

generatedmain=\
	main.aux \
	main.bbl \
	main.blg \
	main.log \
	main.out \
	main.pdf \
	main.spl

main.pdf:
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex main

clean:
	rm -rf $(generatedfigures) $(generatedmain)

